Online Adaptive Policy Selection in Time-Varying Systems: No-Regret via Contractive Perturbations

We study online adaptive policy selection in systems with time-varying costs and dynamics. We develop the Gradient-based Adaptive Policy Selection (GAPS) algorithm together with a general analytical framework for online policy selection via online optimization. Under our proposed notion of contractive policy classes, we show that GAPS approximates the behavior of an ideal online gradient descent algorithm on the policy parameters while requiring less information and computation. When convexity holds, our algorithm is the first to achieve optimal policy regret. When convexity does not hold, we provide the first local regret bound for online policy selection. Our numerical experiments show that GAPS can adapt to changing environments more quickly than existing benchmarks.

==> Proofs/Proof-E-ISS.tex <==
By \Cref{lemma:smooth-multi-step-dynamics}, we see that for any $\tau' \in [\tau: t-1]$, we have
\begin{align}\label{E-ISS:e1}
    &\norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1} + [0_{\times (\tau' - \tau)}, \epsilon_{\tau':t-1}]) - g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1} + [0_{\times (\tau' - \tau + 1)}, \epsilon_{\tau'+1:t-1}])}\nonumber\\
    \leq{}& C_{L, g, \theta} \decayfactor^{t - \tau'} \norm{\epsilon_{\tau'}}.
\end{align}
Therefore, we see that
\begin{subequations}\label{E-ISS:e2}
\begin{align}
    &\norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1}) - g_{t\mid \tau}(x_\tau', \theta_{\tau:t-1} + \epsilon_{\tau:t-1})}\nonumber\\
    \leq{}& \sum_{\tau' = \tau}^{t - 1} \norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1} + [0_{\times (\tau' - \tau)}, \epsilon_{\tau':t-1}]) - g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1} + [0_{\times (\tau' - \tau + 1)}, \epsilon_{\tau'+1:t-1}])}\nonumber\\
    &+ \norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1} + \epsilon_{\tau:t-1}) - g_{t\mid \tau}(x_\tau', \theta_{\tau:t-1} + \epsilon_{\tau:t-1})}\label{E-ISS:e2:s1}\\
    \leq{}& C_{L, g, \theta} \sum_{\tau' = \tau}^{t - 1} \decayfactor^{t - \tau'} \norm{\epsilon_{\tau'}} + C_0 \decayfactor^{t - \tau}\norm{x_\tau - x_\tau'},\label{E-ISS:e2:s2}
\end{align}
\end{subequations}
where we use the triangle inequality in \eqref{E-ISS:e2:s1}; we use \eqref{E-ISS:e1} and the strong exponentially decaying perturbation property in \eqref{E-ISS:e2:s2}.

==> Proofs/Proof-main-regret-bound-convex.tex <==
In this section, we first present \Cref{thm:main-regret-bound-convex} with specific expressions of the bounds in \Cref{thm:main-regret-bound-convex-specific}. Then, we show \Cref{thm:main-regret-bound-convex-specific} using the results we discussed in \Cref{sec:main-proof-outline}.

\begin{theorem}\label{thm:main-regret-bound-convex-specific}
Suppose strong contractive perturbation (\Cref{def:exp-decay-perturbation-property}) holds. Consider GAPS (Algorithm \ref{alg:OCO-with-parameter-update}) with learning rate $\eta_t = \eta$ and buffer size $B$. Let $\{x_t, u_t, \theta_t\}_{t \in [0:T-1]}$ denote the trajectory of Algorithm \ref{alg:OCO-with-parameter-update}. Under Assumption \ref{assump:dynamics-and-policy-class}, the following inequalities hold
\begin{align*}
    \abs{f_t(x_t, u_t) - F_t(\theta_t)}&\leq \frac{C_{L, f, \theta}^2 \rho}{(1 - \rho)^3} \cdot \eta,\\
    \norm{G_t - \nabla F_t(\theta_t)}&\leq \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right) \eta + \frac{C_{L, f, \theta}}{1 - \rho} \cdot \rho^B,
\end{align*}
where the constants $C_{L, f, \theta}, \hat{C}_0, \hat{C}_1, \hat{C}_2$ are given in \Cref{coro:smooth-multi-step-costs} and \Cref{thm:OCO-with-parameter-update-gradient-bias}.
If Assumption \ref{assump:convex-multi-step-cost-function} also holds, the following adaptive regret holds
\begin{align*}
    R^A(T)\leq{}& \left(\frac{C_{L, f, \theta}^2}{(1 - \rho)^3} + \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)D\right)\eta + \frac{D^2}{2\eta T} + \frac{D C_{L, f,\theta}}{1 - \rho} \cdot \rho^B\\
    &+2\left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)^2 D^2 \eta^3 + \frac{2 C_{L, f, \theta}^2}{(1 - \rho)^2}\rho^{2B}\eta.
\end{align*}
Further, if we assume $T >> \frac{1}{1 - \rho}$ and set $\eta = (1 - \rho)^{\frac{5}{2}} T^{-\frac{1}{2}}, B \geq \frac{1}{2} \log(T) /\log(1/\rho)$, the time-averaged adaptive regret is $R^A(T) = O\left((1-\rho)^{-\frac{5}{2}}T^{-\frac{1}{2}}\right)$. {
\color{blue} Further, the time-averaged dynamic regret is upper bounded by
\begin{align*}
    &R^D(T) \leq 2\left(\frac{C_{L, f, \theta}^2}{(1 - \rho)^3} + \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)D\right)\eta + \frac{3 D^2}{\eta T} + \frac{2 D C_{L, f,\theta}}{1 - \rho} \cdot \rho^B\\
    &+4\left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)^2 D^2 \eta^3 + \frac{4 C_{L, f, \theta}^2}{(1 - \rho)^2}\rho^{2B}\eta + \left(\frac{2D}{\eta T} + \frac{C_{L, f, \theta}}{(1 - \rho)^2 T}\right)\sum_{t=1}^{T-1} \norm{\hat{\theta}_t - \hat{\theta}_{t-1}}.
\end{align*}
Further, if we assume $T >> \frac{1}{1 - \rho}$ and set $\eta = (1 - \rho)^{\frac{5}{2}} (\hat{P}/T)^{\frac{1}{2}}, B \geq \frac{1}{2} \log(T) /\log(1/\rho)$, the time-averaged dynamic regret is $R^D(T) = O\left((1-\rho)^{-\frac{5}{2}}(\hat{P}/T)^{\frac{1}{2}}\right)$, where $\hat{P}\coloneqq 1 + \sum_{t=1}^{T-1} \norm{\hat{\theta}_t - \hat{\theta}_{t-1}}$.
}
\end{theorem}

\begin{proof}[Proof of \Cref{thm:main-regret-bound-convex-specific}]
The first two inequalities are shown in \Cref{thm:OCO-with-parameter-update-trajectory-distance} and \Cref{thm:OCO-with-parameter-update-gradient-bias}. Thus, we focus on the adaptive regret part here in the proof.

Fix a time interval $I = [r: s] \subseteq [0: T-1]$ and let $\theta_I$ be an arbitrary policy parameter in $\Theta$. By \Cref{thm:OGD-with-biased-gradient-regret} and \Cref{thm:OCO-with-parameter-update-gradient-bias}, we see that the sequence of policy parameters of the online policy satisfies that
\begin{align}\label{thm:main-regret-bound-convex:e1}
    \frac{1}{T}\left(\sum_{t = r}^{s}F_t(\theta_t) - \sum_{t=r}^{s}F_t(\theta_I)\right) \leq (W^2 + \epsilon^2)\eta + \frac{D^2}{2\eta T} + \epsilon D,
\end{align}
where $W = \frac{C_{L, f,\theta}}{1 - \rho}$ by \Cref{thm:OCO-with-parameter-update-trajectory-distance} and $\epsilon = \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right) \eta + \frac{C_{L, f, \theta}}{1 - \rho} \cdot \rho^B$.

Note that by definition, we have $F_t(\theta_I) = f_t(\hat{x}_t(\theta_I), \hat{u}_t(\theta_I))$ and by \Cref{thm:OCO-with-parameter-update-trajectory-distance}, we have
\begin{align}\label{thm:main-regret-bound-convex:e2}
    \abs{f_t(x_t, u_t) - F_t(\theta_t)} \leq \frac{C_{L, f, \theta}^2 \rho}{(1 - \rho)^3}\cdot \eta.
\end{align}
Substituting these into \eqref{thm:main-regret-bound-convex:e1} gives that
\begin{align*}
    &\frac{1}{T}\left(\sum_{t = r}^{s}f_t(x_t, u_t) - \sum_{t = r}^{s}f_t(\hat{x}_t(\theta_I), \hat{u}_t(\theta_I))\right)\\
    \leq{}& \frac{1}{T}\left(\sum_{t = r}^{s} F_t(\theta_t) - \sum_{t=r}^{s} F_t(\theta_I)\right) + \frac{1}{T}\sum_{t = r}^{s}\abs{f_t(x_t, u_t) - F_t(\theta_t)}\\
    \leq{}& \frac{D^2}{2\eta T} + \epsilon D + \left(W^2 + \epsilon^2 + \frac{C_{L, f, \theta}^2 \rho}{(1 - \rho)^3}\right)\cdot \eta\\
    \leq{}& \left(\frac{C_{L, f, \theta}^2}{(1 - \rho)^3} + \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)D\right)\eta + \frac{D^2}{2\eta T} + \frac{D C_{L, f,\theta}}{1 - \rho} \cdot \rho^B\\
    &+2\left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)^2 D^2 \eta^3 + \frac{2 C_{L, f, \theta}^2}{(1 - \rho)^2}\rho^{2B}\eta,
\end{align*}
where we used \eqref{thm:main-regret-bound-convex:e1} and \eqref{thm:main-regret-bound-convex:e2} in the second inequality.

{\color{blue}
Now we show the dynamic regret bound in \Cref{thm:main-regret-bound-convex:e1}. By \Cref{thm:OGD-with-biased-gradient-regret} and \Cref{thm:OCO-with-parameter-update-gradient-bias}, we see that the sequence of policy parameters of the online policy satisfies that
\begin{align}\label{thm:main-regret-bound-convex:e3}
    \frac{1}{T}\left(\sum_{t=0}^{T-1}F_t(\theta_t) - \sum_{t=0}^{T-1}F_t(\hat{\theta}_t)\right)\leq \frac{3 D^2}{\eta T} + \frac{2D}{\eta T}\sum_{t=1}^{T-1} \norm{\hat{\theta}_t - \hat{\theta}_{t-1}} + \eta (W + \epsilon)^2 + 2 \epsilon D,
\end{align}
where $W = \frac{C_{L, f,\theta}}{1 - \rho}$ by \Cref{thm:OCO-with-parameter-update-trajectory-distance} and $\epsilon = \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right) \eta + \frac{C_{L, f, \theta}}{1 - \rho} \cdot \rho^B$.

Recall that by \Cref{thm:OCO-with-parameter-update-trajectory-distance}, we have that
\begin{align*}
    \abs{f_t(x_t, u_t) - F_t(\theta_t)} \leq{}& \frac{C_{L, f, \theta}^2 \rho}{(1 - \rho)^3}\cdot \eta,\\
    \abs{f_t(\hat{x}_t, \hat{u}_t) - F_t(\hat{\theta}_t)} \leq{}& \frac{C_{L, f, \theta}}{1 - \rho} \sum_{\tau = 0}^{t-1} \rho^\tau \norm{\hat{\theta}_{t-\tau} - \hat{\theta}_{t-\tau-1}}.
\end{align*}
Substituting these into \eqref{thm:main-regret-bound-convex:e3} gives that
\begin{align*}
    &\frac{1}{T}\left(f_t(x_t, u_t) - f_t(\hat{x}_t, \hat{u}_t)\right)\\
    \leq{}& \frac{1}{T}\left(\sum_{t=0}^{T-1}F_t(\theta_t) - \sum_{t=0}^{T-1}F_t(\hat{\theta}_t)\right) + \frac{1}{T}\sum_{t=0}^{T-1} \abs{f_t(x_t, u_t) - F_t(\theta_t)} + \frac{1}{T}\sum_{t=0}^{T-1} \abs{f_t(\hat{x}_t, \hat{u}_t) - F_t(\hat{\theta}_t)}\\
    \leq{}& \frac{3 D^2}{\eta T} + \frac{2D}{\eta T}\sum_{t=1}^{T-1} \norm{\hat{\theta}_t - \hat{\theta}_{t-1}} + \eta (W + \epsilon)^2 + 2 \epsilon D + \frac{C_{L, f, \theta}^2 \rho}{(1 - \rho)^3}\cdot \eta + \frac{C_{L, f, \theta}}{(1 - \rho)T} \sum_{t = 0}^{T-1} \sum_{\tau = 0}^{t-1} \rho^\tau \norm{\hat{\theta}_{t-\tau} - \hat{\theta}_{t-\tau-1}}\\
    \leq{}& 2\left(\frac{C_{L, f, \theta}^2}{(1 - \rho)^3} + \left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)D\right)\eta + \frac{3 D^2}{\eta T} + \frac{2 D C_{L, f,\theta}}{1 - \rho} \cdot \rho^B\\
    &+4\left(\frac{\hat{C}_0}{1 - \rho} + \frac{\hat{C}_1 + \hat{C}_2}{(1 - \rho)^2} + \frac{\hat{C}_2}{(1 - \rho)^3}\right)^2 D^2 \eta^3 + \frac{4 C_{L, f, \theta}^2}{(1 - \rho)^2}\rho^{2B}\eta + \left(\frac{2D}{\eta T} + \frac{C_{L, f, \theta}}{(1 - \rho)^2 T}\right)\sum_{t=1}^{T-1} \norm{\hat{\theta}_t - \hat{\theta}_{t-1}}.
\end{align*}
}
\end{proof}

==> Proofs/Proof-static-to-time-varying.tex <==
We first show that, under a time-invariant policy parameter $\theta$, starting from an arbitrary $x_\tau$ that satisfies $\norm{x_\tau} \leq R_C$, we have $\norm{x_t} \leq R_S + C \rho^{t-\tau} \norm{x_\tau}$ for all $t \geq \tau$.

To see this, note that by time-invariant contractive perturbation, we have
\begin{align*}
    \norm{g_{t\mid \tau}(x_\tau, \theta_{\times (t - \tau)})} \leq{}& \norm{g_{t\mid \tau}(x_\tau, \theta_{\times (t - \tau)}) - g_{t\mid \tau}(0, \theta_{\times (t - \tau)})} + \norm{g_{t\mid \tau}(0, \theta_{\times (t - \tau)})}\\
    \leq{}& C \rho^{t - \tau}\norm{x_\tau} + R_S.
\end{align*}

Now, we show that if starting from $x_\tau$ that satisfies, the trajectory induced by an $\hat{\varepsilon}$-time-varying parameter sequence satisfies that $\norm{x_t} \leq \hat{R}_S + C \rho^{t - \tau} \norm{x_\tau}$ for all $t \geq \tau$. Since this ball is contained in $B(0, R_C)$, we know the time-invariant contractive perturbation always apply.

We show this statement by induction. Suppose the statement holds for all time steps $\tau, \ldots, t - 1$. We see that
\begin{align*}
    &\norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1}) - g_{t\mid \tau}(x_\tau, \theta_{\times (t - \tau)})}\\
    \leq{}& \sum_{j = \tau}^{t}\norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:j}, (\theta_t)_{\times (t - j-1)}) - g_{t\mid \tau}(x_\tau, \theta_{\tau:j-1}, (\theta_t)_{\times (t - j)})}\\
    \leq{}& C L_{g, u}(B_0) L_{\pi, \theta}(B_0) \sum_{j = \tau}^t \rho^{t - j - 1} \norm{\theta_t - \theta_j} \leq \frac{C L_{g, u}(B_0) L_{\pi, \theta}(B_0) \hat{\epsilon}}{(1 - \rho)^2}.
\end{align*}
Therefore, we see that
\begin{align*}
    \norm{g_{t\mid \tau}(x_\tau, \theta_{\tau:t-1})} \leq{}& \norm{g_{t\mid \tau}(x_\tau, \theta_{\times (t - \tau)})} + \frac{C L_{g, u}(B_0) L_{\pi, \theta}(B_0) \hat{\epsilon}}{(1 - \rho)^2}\\
    \leq{}& C \rho^{t-\tau} \norm{x_\tau} + R_S + \frac{C L_{g, u}(B_0) L_{\pi, \theta}(B_0) \hat{\epsilon}}{(1 - \rho)^2}\\
    ={}& C \rho^{t - \tau} \norm{x_\tau} + \hat{R}_S.
\end{align*}
This finishes the proof of $\varepsilon$-time-varying stability.



==> Proofs/Proof-weak-to-strong-adaptive-stability.tex <==
Since contractive perturbation holds for $(C, \rho)$, we see that
\begin{subequations}\label{lemma:strong-adaptive-stability:e1}
\begin{align}
    \norm{\hat{x}_t - \bar{x}_t} ={}&\norm{g_{t\mid 0}(x_0, \hat{\theta}_{0:t-1}) - g_{t\mid 0}(x_0, \bar{\theta}_{\times t})}\nonumber\\
    \leq{}& \sum_{\tau = 0}^{t-1} \norm{g_{t\mid 0}(x_0, \hat{\theta}_{0:\tau-1}, \bar{\theta}_{\times (t - \tau)}) - g_{t\mid 0}(x_0, \hat{\theta}_{0:\tau}, \bar{\theta}_{\times (t - \tau - 1)})}\label{lemma:strong-adaptive-stability:e1:s1}\\
    \leq{}& \sum_{\tau = 0}^{t-1} \norm{g_{t\mid \tau+1}(g_{\tau+1\mid\tau}(\hat{x}_\tau, \bar{\theta}), \bar{\theta}_{\times (t - \tau - 1)}) - g_{t\mid \tau+1}(g_{\tau+1\mid\tau}(\hat{x}_\tau, \hat{\theta}_\tau), \bar{\theta}_{\times (t - \tau - 1)})}\label{lemma:strong-adaptive-stability:e1:s2}\\
    \leq{}& C \sum_{\tau = 0}^{t-1} \rho^{t-\tau-1} \norm{g_{\tau+1\mid\tau}(\hat{x}_\tau, \bar{\theta}) - g_{\tau+1\mid\tau}(\hat{x}_\tau, \hat{\theta}_\tau)}\label{lemma:strong-adaptive-stability:e1:s3}\\
    \leq{}& C L_{\ALG, \theta} L_{g, x} \sum_{\tau=0}^{t-1}\rho^{t - \tau - 1}\norm{\hat{\theta}_{\tau} - \bar{\theta}},\label{lemma:strong-adaptive-stability:e1:s4}
\end{align}
\end{subequations}
where we use the triangle inequality in \eqref{lemma:strong-adaptive-stability:e1:s1}; we use the definition of multi-step dynamics (\Cref{def:multi-step-dynamics}) and the notation $\hat{x}_\tau \coloneqq g_{\tau\mid 0}(x_0, \hat{\theta}_{0:\tau-1})$ in \eqref{lemma:strong-adaptive-stability:e1:s2}; we use the assumption that contractive perturbation (\Cref{def:exp-decay-perturbation-property}) holds with $(C, \rho)$ in \eqref{lemma:strong-adaptive-stability:e1:s3}; we use the Lipschitzness of $g_\tau$ and $\ALG_\tau$ given by \Cref{assump:dynamics-and-policy-class-a} in \eqref{lemma:strong-adaptive-stability:e1:s4}.

Since $\ALG_t$ is $(L_{\ALG, x}, L_{\ALG, \theta})$-Lipschitz on $\mathcal{X} \times \Theta$, we see that
\begin{subequations}\label{lemma:strong-adaptive-stability:e2}
\begin{align}
    \norm{\hat{u}_t - \bar{u}_t} ={}& \norm{\ALG_t(\hat{x}_t, \hat{\theta}_t) - \ALG_t(\bar{x}_t, \bar{\theta})}\nonumber\\
    \leq{}& L_{\ALG, x} \norm{\hat{x}_t - \bar{x}_t} + L_{\ALG, \theta} \norm{\hat{\theta}_t - \bar{\theta}}\label{lemma:strong-adaptive-stability:e2:s1}\\
    \leq{}& C L_{\ALG, x} L_{\ALG, \theta} L_{g, x} \sum_{\tau=0}^{t-1}\rho^{t - \tau - 1}\norm{\hat{\theta}_{\tau} - \bar{\theta}} + L_{\ALG, \theta} \norm{\hat{\theta}_t - \bar{\theta}}, \label{lemma:strong-adaptive-stability:e2:s2}
\end{align}
\end{subequations}
where we use \Cref{assump:dynamics-and-policy-class-a} in \eqref{lemma:strong-adaptive-stability:e2:s1}; we use \eqref{lemma:strong-adaptive-stability:e1} in \eqref{lemma:strong-adaptive-stability:e2:s2}.


==> numerical-quadrotor.tex <==
\label{sec:quadrotor}
\james{Writing this late at night... writing style is not polished yet.}
In this example, we evaluate \Cref{alg:OCO-with-parameter-update} on a nonlinear dynamical system.
We consider a quadrotor helicopter delivering a sequence of $P$ dissimilar packages.
We model this as a sequence of step changes in the quadrotor's mass and inertia matrix.

In this section we will refer to the distribution of a random variable whose logarithm is uniformly distributed by the notation $G(\mu, p)$ for $p \geq 0$, so if $z \sim G(\mu, p)$ then $z = \mu p^s,\ s \sim U[-1, 1]$.

The quadrotor has a nominal mass $m^\nom$ and diagonal inertia matrix $I^\nom$.
Each package induces the mass $m^j$ and inertia $I^j$ for $j \in \{1, \dots, P\}$.
We sample $m^j \sim G(m_\nom, 2)$.
The three eigenvalues of an inertia matrix must satisfy the triangle inequality $\lambda_1 + \lambda_2 \geq \lambda_3$ in all permutations.
To generate random inertia matrices, we sample diagonal matrices according to
$I_{i,i} \sim G(I^\nom_{i,i}, 4)$ and perform rejection sampling to enforce the triangle inequalities.

Mass is easy to measure, so we assume the availability of an approximate estimate of the current mass $\widehat m^j \sim G(m^j, 1.2)$.
However, inertia is harder to estimate.
Therefore, we simulate the heuristic estimate
$\widehat I^j = (\widehat m^j / m^\nom) I^\nom$.

The quadrotor must track a trajectory given by $\{p^d_t\}_{t=1}^T \in (\bR^3)^T$
with a known derivative $\dot p^d_t$.
The quadrotor's state is defined by
$x_t = (p_t, v_t, R_t, \omega_t)$,
where $p_t \in \bR^3$ is the position,
$v_t \in \bR^3$ is the linear velocity,
$R_t \in \operatorname{SO}(3)$ is the rotation from world coordinates to body coordinates,
and $\omega_t \in \bR^3$ is the angular velocity in body coordinates.
The control inputs $u \in \bR_+^4$ are the thrust outputs of the four rotors.
The cost function is given by
$f_t(x_t, u_t) = \norm{p_t}^2 + \alpha \norm{u_t}^2$,
where $\alpha \ll 1$ prioritizes position tracking error at the cost of control energy.

The ``context'' information known by the policy when carrying package $j$ at time $t$ is thus
$y_t = (\hat m^j, \hat I^j, p^d_t, \dot p^d_t)$.

We consider the quadrotor following the dynamics model and geometric tracking policy of \citet{lee2010geometric}.
For the sake of brevity, we omit the equations of motion and the exact form of the policy here.
The policy is parameterized by four positive feedback gain constants
$\theta = (k_p, k_v, k_R, k_\omega)$
relating to position, velocity, attitude, and angular velocity tracking errors, respectively.
Intuitively, the policy can be understood as a ``PD policy on a manifold''.

We emphasize that this system is nonlinear and does not satisfy the assumptions of our regret bound.
\todo{appeal to gradient estimate guarantee}.
The purpose of this simulation is to investigate if our method still behaves well on such a system in practice.

We deploy our method on the simulated quadrotor with $P = 20$ packages.
The continuous-time dynamics are discretized with forward Euler integration over a time step of $1/200$ second.
The total time is $T = 20000$ with the time divided unequally between the packages.
The tracking trajectory $p^d_t$ is specified by a circle with a period of $10$ seconds and a radius of $2$ meters.

\begin{figure}
    \hfill \includegraphics[width=0.974\textwidth]{figures/quadrotor_pid_traces.pdf}
    \includegraphics[width=\textwidth]{figures/quadrotor_z.pdf}
    \caption{
        Results of GAPS in the nonlinear quadrotor package delivery scenario (\Cref{sec:quadrotor}).
        \emph{Top}: Evolution of policy gain parameters selected by our method.
        To account for varying scales, the ratios of the chosen parameters to their initial values are plotted.
        \emph{Bottom}: Altitude component of trajectory tracking error.
        Desired altitude is zero.
        Errors in mass estimates $\widehat m^j$ prevent zero tracking error.
        \james{Would make more sense to plot LQR cost?.}
        \james{Could plot the random-search approximate fixed $\theta^\star$ also.}
    }
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \includegraphics[width=0.4\textwidth]{figures/quadrotor_xy.pdf}
    \hfill
    \raisebox{6mm}{\includegraphics[width=0.45\textwidth]{figures/quadrotor_regret.pdf}}
    \caption{
        More results of GAPS in the nonlinear quadrotor package delivery scenario (\Cref{sec:quadrotor}).
        \emph{Left}: Tracking performance in the horizontal plane.
        The cycles with larger error are at the beginning of the simulation.
        \emph{Right:} Approximate ``regret'' computed by comparison to a random search. \todo{details}
    }
    \label{fig:my_label}
\end{figure}

==> tikz/multistep.tex <==
\begin{tikzpicture}[
	xscale=0.7,
	yscale=0.5,
	nodex/.style={draw},
	nodeu/.style={circle, inner sep=0.7mm, draw},
	nodeth/.style={diamond, inner sep=0.3mm, draw},
	nodez/.style={diamond, inner sep=0.3mm, draw},
	edge/.style={-Straight Barb},
	baseline=(x0),
]
    \node[nodex] (x0) at (-3, -2) {$x_0$};
    \node[nodex] (x1) at (0, -2) {$x_1$};
	\node[nodex] (x2) at (2, -2) {$x_2$};
	\node[nodex] (x3) at (4, -2) {$x_3$};
	\node (x4) at (6, -2) {$\dots$};
 \node[nodex] (x5) at (8.5, -2) {$x_{\tau-1}$};
 \node[nodex] (x6) at (11, -2) {$x_\tau$};
	\node[nodeu] (u0) at (0, 0.25) {$F_1$};
	\node[nodeu] (u1) at (2, 0.25) {$F_2$};
	\node[nodeu] (u2) at (4, 0.25) {$F_3$};
	\node (u5) at (6, 0.25) {$\hdots$};
	\node[nodeu] (u3) at (8.5, 0.25) {$F_{\tau-1}$};
	\node[draw, rounded corners] (u4) at (11.5, 0.35) {$F_{\tau}(\theta)$};
	\node[nodeth] (th0) at (-1.5, -4.25) {$\theta_0$};
    \node[nodeth] (th1) at (0, -4.25) {$\theta_1$};
	\node[nodeth] (th2) at (2, -4.25) {$\theta_2$};
	\node[nodeth] (th3) at (4, -4.25) {$\theta_3$};
	\node (blank) at (6, -4.25) {$\hdots$};
    \node[nodeth] (th4) at (8.5, -4.25) {$\theta_{\tau-1}$};
    \node[nodeth] (th5) at (11, -4.25) {$\theta_\tau$};
	\node[nodeth, inner sep=0.8mm] (th) at (-3, -6) {$\theta$};

	\draw[edge] (x1) -- (u0);
	\draw[edge] (x2) -- (u1);
	\draw[edge] (x3) -- (u2);
	\draw[edge] (x3) -- (x4);
    \draw[edge] (x4) -- (x5);
    \draw[edge] (x4) -- (u5);
    \draw[edge] (blank) -- (x4);
    \draw[edge] (x5) -- (x6);

	\draw[edge] (th) -| (th0);
	\draw[edge] (th) -| (th1);
	\draw[edge] (th) -| (th2);
	\draw[edge] (th) -| (th3);
	\draw[edge] (th) -| (th4);
	\draw[edge] (th) -| (blank);
    \draw[edge] (th) -| (th5);


	\draw[edge] (x0) edge["$g_0$"] (x1);
	\draw[edge] (x1) edge["$g_1$"] (x2);
	\draw[edge] (x2) edge["$g_2$"] (x3);
	\draw[edge] (x3) edge["$g_3$"] (x4);
	\draw[edge] (x4) edge["$g_{\tau-2}$"] (x5);
	\draw[edge] (x5) edge["$g_{\tau-1}$"] (x6);

	\draw[edge] (th0) -- (x1);
	\draw[edge] (th1) -- (x1);
	\draw[edge] (th2) -- (x2);
	\draw[edge] (th3) -- (x3);
	\draw[edge] (th4) -- (x5);
	\draw[edge] (th5) -- (x6);
	\draw[edge] (x5) -- (u3);
	\draw[edge] (x6) -- (u4);



	\begin{scope}[opacity=0.5]
		\draw[rounded corners, blue!20!white, line width=40pt]
			([yshift=-1mm]x1.center) --
			([yshift=-1mm]x6.center) --
			(u3.center) --
			(u0.center) --
			cycle;
	\end{scope}
\end{tikzpicture}


==> tikz/multistepv2.tex <==
\begin{tikzpicture}[
	xscale=0.7,
	yscale=0.5,
	nodex/.style={draw},
	nodeu/.style={circle, inner sep=0.7mm, draw},
	nodeth/.style={diamond, inner sep=0.3mm, draw},
	edge/.style={-Straight Barb},
	baseline=(x0),
]
	\node[nodex] (x0) at (0, 0) {$x_0$};
	\node[nodex] (x1) at (2, 0) {$x_1$};
	\node[nodex] (x2) at (4, 0) {$x_2$};
	\node[nodex] (x3) at (5.5, 0) {$x_3$};
    \node (x3dots) at (7, 0) {$\dots$};
	\node[nodex] (x4) at (8.5, 0) {$x_{\tau-1}$};
	\node[nodex] (x5) at (10, 0) {$x_{\tau}$};
	\node[nodeu] (u0) at (1, -2) {$u_0$};
	\node[nodeu] (u1) at (3, -2) {$u_1$};
	\node[nodeu] (u2) at (5, -2) {$u_2$};
    \node (u3) at (7, -2) {$\dots$};
	\node[nodeu] (u4) at (9, -2) {$u_{\theta-1}$};
	\node[nodeu] (u5) at (11, -2) {$u_\tau$};
	\node[nodeth] (th0) at (1, -4.5) {$\theta_0$};
	\node[nodeth] (th1) at (3, -4.5) {$\theta_1$};
	\node[nodeth] (th2) at (5, -4.5) {$\theta_2$};
    \node (th3) at (7, -4.5) {$\dots$};
	\node[nodeth] (th4) at (9, -4.5) {$\theta_{\tau-1}$};
	\node[nodeth] (th5) at (11, -4.5) {$\theta_\tau$};
	\node[nodeth, inner sep=0.8mm] (th) at (-1, -6) {$\theta$};
	\node[draw, rounded corners] (cost) at (12, 1.5) {$F_\tau(\theta)$};

	\draw[edge] (th0) -- (u0);
	\draw[edge] (th1) -- (u1);
	\draw[edge] (th2) -- (u2);
	\draw[edge] (th3) -- (u3);
	\draw[edge] (th4) -- (u4);
	\draw[edge] (th5) -- (u5);


	\draw[edge] (u0) -- (x1);
	\draw[edge] (u1) -- (x2);
	\draw[edge] (u2) -- (x3);
	\draw[edge] (u3) -- (x4);
	\draw[edge] (u4) -- (x5);


	\draw[edge] (x0) -- (x1);
	\draw[edge] (x1) -- (x2);
	\draw[edge] (x2) -- (x3);
	\draw[edge] (x3) -- (x3dots);
	\draw[edge] (x3dots) -- (x4);
	\draw[edge] (x4) -- (x5);


	\draw[edge] (x0) -- (u0);
	\draw[edge] (x1) -- (u1);
	\draw[edge] (x2) -- (u2);
	\draw[edge] (x3) -- (u3);
	\draw[edge] (x4) -- (u4);
	\draw[edge] (x5) -- (u5);


	\draw[edge] (th) -| (th0);
	\draw[edge] (th) -| (th1);
	\draw[edge] (th) -| (th2);
	\draw[edge] (th) -| (th3);
	\draw[edge] (th) -| (th4);
	\draw[edge] (th) -| (th5);

	\draw[edge] (x5) -- (cost);
	\draw[edge] (u5) -- (cost);

	\begin{scope}[transparency group, opacity=0.5]
		\draw[rounded corners, fill, VioletRed!30!white, line width=35pt]
			([yshift=-2mm]x0.center) --
			([yshift=-2mm]x5.center) --
			(u5.center) --
			(th5.center) --
			(th0.center) --
			cycle;
	\end{scope}
\end{tikzpicture}


==> tikz/radius_illustration.tex <==
\begin{tikzpicture}
    \draw[-latex] (0, 0) -- (13, 0);
    
    \filldraw[black] (0,0) circle (2pt) node[anchor=north]{$0$};
    \filldraw[black] (2,0) circle (2pt) node[anchor=north]{$R_S$};
    \filldraw[blue] (5,0) circle (2pt) node[anchor=south]{$R_S + C \norm{x_0}$};
    \filldraw[black] (7,0) circle (2pt) node[anchor=north]{$R_C$};
    \filldraw[blue] (9.5,0) circle (2pt) node[anchor=south]{$C(R_S + C \norm{x_0}) + R_S$};
    \filldraw[black] (12,0) circle (2pt) node[anchor=north]{$R_x$};

\end{tikzpicture}

==> tikz/surrogate.tex <==
\begin{tikzpicture}[
	xscale=0.7,
	yscale=0.5,
	nodex/.style={draw},
	nodeu/.style={circle, inner sep=0.7mm, draw},
	nodeth/.style={diamond, inner sep=0.3mm, draw},
	edge/.style={-Straight Barb},
	baseline=(x0),
]
	\node[nodex] (x0) at (0, 0) {$x_0$};
	\node[nodex] (x1) at (2, 0) {$x_1$};
	\node[nodex] (x2) at (4, 0) {$x_2$};
	\node[nodeu] (u0) at (1, -2) {$u_0$};
	\node[nodeu] (u1) at (3, -2) {$u_1$};
	\node[nodeu] (u2) at (5, -2) {$u_2$};
	\node[nodeth] (th0) at (1, -4) {$\theta_0$};
	\node[nodeth] (th1) at (3, -4) {$\theta_1$};
	\node[nodeth] (th2) at (5, -4) {$\theta_2$};

	\node[nodeth, inner sep=0.8mm] (th) at (-1, -5.5) {$\theta$};
	\node[draw, rounded corners] (cost) at (5.5, 1.5) {$F_2(\theta)$};

	\draw[edge] (th0) -- (u0);
	\draw[edge] (th1) -- (u1);
	\draw[edge] (th2) -- (u2);

	\draw[edge] (u0) -- (x1);
	\draw[edge] (u1) -- (x2);

	\draw[edge] (x0) -- (x1);
	\draw[edge] (x1) -- (x2);

	\draw[edge] (x0) -- (u0);
	\draw[edge] (x1) -- (u1);
	\draw[edge] (x2) -- (u2);

	\draw[edge] (th) -| (th0);
	\draw[edge] (th) -| (th1);
	\draw[edge] (th) -| (th2);

	\draw[edge] (x2) -- (cost);
	\draw[edge] (u2) -- (cost);

	\begin{scope}[transparency group, opacity=0.5]
		\draw[rounded corners, fill, VioletRed!30!white, line width=35pt]
			([yshift=-2mm]x0.center) --
			([yshift=-2mm]x2.center) --
			(u2.center) --
			(th2.center) --
			(th0.center) --
			cycle;
	\end{scope}
\end{tikzpicture}

